Reinforcement Learning of POMDPs using Spectral Methods

We propose a new reinforcement learning algorithm for partially observable Markov decision processes (POMDP) based on spectral decomposition methods. While spectral methods have been previously employed for consistent learning of (passive) latent variable models such as hidden Markov models, POMDPs are more challenging since the learner interacts with the environment and possibly changes the future observations in the process. We devise a learning algorithm running through episodes, in each episode we employ spectral techniques to learn the POMDP parameters from a trajectory generated by a fixed policy. At the end of the episode, an optimization oracle returns the optimal memoryless planning policy which maximizes the expected reward based on the estimated POMDP model. We prove an order-optimal regret bound with respect to the optimal memoryless policy and efficient scaling with respect to the dimensionality of observation and action spaces.

==> Cextension.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LIMITED MEMORY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Extension to Bounded-Memory Policies}\label{app:bounded.memory}

\begin{figure}[h]
\tiny
\begin{center}
\begin{psfrags}
\psfrag{x1}[][1]{$x_0$}
\psfrag{x2}[][1]{$x_{1}$}
\psfrag{x3}[][1]{$x_{2}$}
\psfrag{x0}[][1]{$x_{-1}$}
\psfrag{y1}[][1]{$\vecy_0$}
\psfrag{y2}[][1]{$\vecy_{1}$}
\psfrag{y0}[][1]{$\vecy_{-1}$}
\psfrag{r1}[][1]{$r_0$}
\psfrag{r2}[][1]{$r_{1}$}
\psfrag{r0}[][1]{$r_{-1}$}
\psfrag{a1}[][1]{$a_{0}$}
\psfrag{a2}[][1]{$a_{1}$}
\psfrag{a0}[][1]{$a_{-1}$}
\includegraphics[width=0.45\textwidth,natwidth=810,natheight=642,trim={0 1.5cm 2cm 0.5cm},clip]{figs/I-6.eps}
\end{psfrags}
\end{center}
\caption{Bounded-Memory POMDP when \past=2.}
\label{fig:I-6}
\end{figure}


Throughout the paper we consider memory-less policies which only consider the current observation to decide which action to take. Nonetheless, our method, and notably the process of estimation of the POMDP parameters, can be easily extended to the case of bounded-memory policies. Let $\pi$ be a policy such that at time $t$ all the past $\past$ observations are considered to decide the action, that is $f_\pi(a|\vec{y}_t, \vec{y}_{t-1},\ldots,\vec{y}_{t-\past})$. In Fig.~\ref{fig:I-6} we illustrate the case for $\past=2$. In this case, we have to redefine the notion of views that we introduced in Sect.~\ref{s:learning.pomdp}. We define the first view $(\vecy_{-(\past-1)},a_{-(\past-1)},r_{-(\past-1)},\ldots,\vecy_{(-1)},a_{(-1)},r_{(-1)})$, the second view $(\vecy_0,r_0)$, and the third view $(\vecy_{(1)},r_{(1)},\ldots,\vecy_{(\past-1)},r_{(\past-1)})$. Given state $x_0$ and all actions $a_0,\ldots,a_{\past-1}$, it is easy to see that these views are independent and the multi-view model can be applied by extending the definitions of $V_{\nu}^{(l)}$ to this case. If the views satisfy the assumption of being full column rank, then all the results presented in Sect.~\ref{s:learning.pomdp} can be easily extended.




Usually, in the real systems, the agents do not make decision at each time step, even they do not apply their decision at each time step because usually making decision and applying that is expensive for agents. Lets take a look at the system that the agent chooses an action based on $p$ previous observation (including current observation) and then for $p-1$ time step, it just looks at the system and records the data, after that, based on this collected data, it choose new action. This model is simpler that the above mentioned model which we are not able to investigate it in this draft.  The simpler model is as follow. Let us consider the case of $p=2$, then
\begin{equation}
\begin{split}
&[\obs_1^{a_0=i}]_{l,f}=Pr(\vecy_{-1}=\vec{e}_j,r_{-1}=\vec{e}_b,a_{-1}=c|x_0=f)\\
&[\obs_2^{a_0=i}]_{l,f}=Pr(\vecy_0=\vec{e}_{j'},r_0=\vec{e}_{b'}|x_0=f,a_0=i)\\
&[\obs_3^{a_2=i}]_{l,f}=Pr(\vecy_1=\vec{e}_j,r_1=\vec{e}_b|x_0=f,a_0=i)
\end{split}
\end{equation}
The full rank condition is satisfied if either $\obs$ matrix or $R$ matrix is full column rank and transition matrix is full rank. Same idea as before, the agent do the learning part for each action and for each of them once it looks at third view as a third effect and once second view as a third view. By this it can learn $\obs$ and $\trans^{(a_0=i)}$ for all $i$. Addition to that, the agent need to find out the transition matrix when during passive time which is for example transition form $x_{-1}$ to $x_0$. To learn this part of model, the agent needs to estimate another set of $\obs$ matrices whose columns are conditioned on $x_1$, $i.e.$:
\begin{equation}
\begin{split}
&[\obs_1]_{l,f}=Pr(\vecy_{0}=\vec{e}_j,r_{0}=\vec{e}_b,a_{0}=c|x_1=f)\\
&[\obs_2]_{l,f}=Pr(\vecy_1=\vec{e}_{j'},r_1=\vec{e}_{b'}|x_1=f)\\
&[\obs_3]_{l,f}=Pr(\vecy_2=\vec{e}_j,r_2=\vec{e}_b,a_2=c|x_1=f)
\end{split}
\end{equation}
this set of $\obs$ gives us the transition matrix.




==> Table.tex <==
\section{Table of Content}
\begin{table}[htbp]\caption{Table of Notation My Research}
\begin{center}% used the environment to augment the vertical space
% between the caption and the table
\begin{tabular}{r c p{10cm} }
\toprule

$\X$ &  & Finite state space \\
$\Y$ &  & Finite observation space\\ 
$\A$ &  & Finite action space \\  
$\R$ &  & Finite reward space\\  
$X$ &  & Cardinality of state space\\  
$Y$ &  & Cardinality of observation space\\  
$A$ &  & Cardinality of action space\\  
$R$ &  & Cardinality of reward space\\  
$r_{\max}$ &  & Largest reward\\  
$x$ &  & state indicator random variable\\  
$\vec{y}$ &  & observation indicator random variable\\  
$r$ &  & reward indicator random variable\\
$a~or~l$ &  & action indicator random variable\\    
$T$ &  & Transition tensor \\  
$O$ &  & Observation matrix\\  
$\Gamma$ &  & Reward tensor\\
$\Pi$ &  & Policy matrix\\
$M$ &  & POMDP model\\
$\M^{(k)}$ &  & Set of plausible POMDP at episode $k$\\
$f_T(x'|x,a)$ &  & transition density from state $x$ to state $x'$ given action $a$\\  
$f_O(\vec{y}|x)$ &  & observation density\\  
$f_R(r|x,a)$ &  & reward density given pair of state-action\\  
$f_T(x'|x)$ &  & corresponding Markov chain transition density\\  
$\widehat{f}_T(x'|x,a)$ &  & transition density from state $x$ to state $x'$ given action $a$\\  
$\widehat{f}_O(\vec{y}|x)$ &  & observation density\\  
$\widehat{f}_R(r|x,a)$ &  & reward density given pair of state-action\\  
$\widehat{f}_T(x'|x)$ &  & corresponding Markov chain transition density\\  
$\calP$ &  & Set of all plausible stochastic memory-less policies\\  
$\pi$ &  & memory less policy, observation $\rightarrow$ action\\  
$\pi_min$ &  & smallest element of policy matrix memory less policy, observation $\rightarrow$ action\\  
$\eta(\pi,M)$ &  & expected average reward given model and policy\\ 
$\eta^+$ &  & expected average reward given model and best memory-less policy\\   
$\omega_\pi$ &  & vector of stationary distribution over states given policy $\pi $ \\  
$\omega_\pi^l$ &  & vector of stationary distribution over states given policy $\pi $ given middle action $l$ \\ 







\bottomrule
\end{tabular}
\end{center}
\label{tab:TableOfNotationForMyResearch1}
\end{table}







\begin{table}[htbp]\caption{Table of Notation My Research}
\begin{center}% used the environment to augment the vertical space
% between the caption and the table
\begin{tabular}{r c p{10cm} }
\toprule
$\bar{r}_\pi(x)$ &  & average reward at state $x$ given\\  
$\pi^+$ &  & best stochastic memory-less policy\\  
$\vec{v}_{i,t}^{(l)}$ &  & $i'th$ view at time t give $a_t=l$(middle action= $l$), $i\in\{1,2,3\}$\\  
$V_{\nu}^{(l)}$ &  & $\nu'th$ View matrix representation $\nu\in\{1,2,3\}$\\  
$\widehat{V}_{\nu}^{(l)}$ &  & $\nu'th$ Estimated view matrix representation $\nu\in\{1,2,3\}$\\  
$K_{\nu,\nu'}^{(l)}$ &  & Covariance matrix between view $\nu$ and $\nu'$, where $\nu,nu'\in\{1,2,3\}$ given middle action $l$\\  
$K^{\dagger}$ &  & Pseudo inverse of matrix K\\  
$M_2^{(l)}$ &  & Second order moment given middle action $l$\\  
$M_3^{(l)}$ &  & Third order moment given middle action $l$\\
$\widehat{M}_2^{(l)}$ &  & Empirical estimate of second order moment given middle action $l$\\  
$\widehat{M}_3^{(l)}$ &  & Empirical estimate of third order moment given middle action $l$\\
$\widehat{M}^{(k)}_2{(l)}$ &  & Empirical estimate of second order moment given middle action $l$ at episode $k$\\  
$\widehat{M}_3^{(k)}{(l)}$ &  & Empirical estimate of third order moment given middle action $l$ at episode $k$\\
$\mu_{\nu,i}^{(l)}$ &  & $i'th$ column of $V_{\nu}^{(l)}$ \\  
$\sigma_{\nu,\nu'}^{(l)}$ &  & smallest non-zero singular value of covariance matrix of views $\nu$ and $\nu'$ given middle action $l$ \\  
$C_O, C_R, C_T$ &  & Suitable numerical constants\\  
$N$ &  & Number of total samples\\  
$N(l)$ &  & Number of triple with middle action $l$\\  
$\lambda^{(l)}$ &  & numerical constant at episode \\  
$C_O^{(k)}, C_R{(k)}, C_T{(k)}$ &  & Suitable numerical constants at episode $k$\\  
$N{(k)}$ &  & Number of samples at episode $k$\\  
$N(l)^{(k)}$ &  & Maximum number of triple with middle action $l$ up episode $k$\\  
$\lambda^{(k)}{(l)}$ &  & numerical constant $k$\\  
$\tilde{\pi}^{k)}$ &  & optimistic policy at episode $k$\\  
$\nu^{(k)}(l)$ &  & Number of triple with middle action $l$ at episode $k$\\  
$D$ &  & The model diameter\\  
$t_{mix}$ &  & mixing time\\  
$Reg_{N}$ &  & Regret up to step $N$\\  
$\rho$ &  & auxiliary parameter in learning algorithm\\  
$\B_O$ &  & Upper confidence bound over error of estimated $f_O$\\  
$\B_R$ &  & Upper confidence bound over error of estimated $f_R$\\  
$B_T$ &  & Upper confidence bound over error of estimated $f_T$\\  
$\psi$ &  & Burn-in time\\  
\bottomrule
\end{tabular}
\end{center}
\label{tab:TableOfNotationForMyResearch2}
\end{table}









\begin{table}[htbp]\caption{Table of Notation My Research}
\begin{center}% used the environment to augment the vertical space
% between the caption and the table
\begin{tabular}{r c p{10cm} }
\toprule
$\Delta_{n^{(l)}}$ &  & Concentration matrix\\  
$\eta_{i,j}^{(l)}(\cdot,\cdot,\cdot)$ &  & mixing coefficient\\  
$p(i,l)$ &  & translator of $i'th$ element in sequence of samples given middle action $l$ to the actual sequence number \\  
$\HH^{i|l}$ &  & $i'th$ quadruple consequence of states random variable given second action $l$\\  
$\hhh^{i|l}$ &  & $i'th$ quadruple consequence of states given second action $l$\\  
$\HH^{j|l}_i$ &  & sequence of all $\HH^{i'|l}$ for $i'\in\{i,\ldots,j\}$ \\  
$\hhh^{i|l}$ &  & sequence of all $\hhh^{i'|l}$ for $i'\in\{i,\ldots,j\}$\\  
$\VV^{i|l}$ &  & $i'th$ triple consequence of views random variable given second action $l$\\  
$\vv^{i|l}$ &  & $i'th$ triple consequence of observation given second action $l$\\  
$\VV^{j|l}_i$ &  & sequence of all $\VV^{i'|l}$ for $i'\in\{i,\ldots,j\}$ \\  
$\vv^{i|l}$ &  & sequence of all $\vv^{i'|l}$ for $i'\in\{i,\ldots,j\}$\\  
$T$ &  & T\\  
$T$ &  & T\\  
$T$ &  & T\\  
$T$ &  & T\\  
$T$ &  & T\\  
$T$ &  & T\\ 
$T$ &  & T\\  
$T$ &  & T\\ 
$T$ &  & T\\  
$T$ &  & T\\
$T$ &  & T\\  
$T$ &  & T\\ 
$T$ &  & T\\  
$T$ &  & T\\ 


\multicolumn{3}{c}{}\\
\multicolumn{3}{c}{\underline{Decision Variables}}\\
\multicolumn{3}{c}{}\\
$y_f$ & $=$ & \(\left\{\begin{array}{rl}
1,  & \text{if Supplier located at site $f$ is open} \\
0,  & \text{otherwise} \end{array} \right.\)\\
\bottomrule
\end{tabular}
\end{center}
\label{tab:TableOfNotationForMyResearch3}
\end{table}


==> macros.tex <==

%\mbox - function definitions
\def\tl{\tilde}\renewcommand\t{{\scriptscriptstyle\top}}

\newcommand\Dir{\operatorname{Dir}}
\newcommand\inner[1]{\ensuremath{\langle #1 \rangle}}
%\newcommand{\aacomment}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# AA:} \textsf{#1} \#\#\#}}}
\newcommand{\mjcomment}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# MJ:} \textsf{#1} \#\#\#}}}
\newcommand{\hscomment}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# HS:} \textsf{#1} \#\#\#}}}
\def\indicator{{1{\hskip -2.5 pt}\hbox{I}}}
\DeclareMathOperator{\polylog}{polylog}
\newcommand\cov{\operatorname{Cov}}
 %\DeclareMathOperator{\short}{short}
\DeclareMathOperator{\sym}{Sym}
  \DeclareMathOperator{\tw}{tw}
  \DeclareMathOperator{\local}{local}
  \DeclareMathOperator{\range}{range}
   \DeclareMathOperator{\Path}{Path}
 \DeclareMathOperator{\Sg}{Sg}
 \DeclareMathOperator{\spt}{SP}
 \DeclareMathOperator{\avg}{avg}
  \DeclareMathOperator{\nbd}{\mathcal{N}}
 \DeclareMathOperator{\parent}{Pa}
 \DeclareMathOperator{\Cq}{Cq}
 \DeclareMathOperator{\TW}{TW}
 

 \DeclareMathOperator{\approxML}{ApproxML}
 \DeclareMathOperator{\Bethe}{Bethe}
 \DeclareMathOperator{\TRW}{TRW}
 \DeclareMathOperator{\conv}{Conv}
 \DeclareMathOperator{\lbp}{LBP}
 \DeclareMathOperator{\Corr}{Corr}
 \DeclareMathOperator{\hCorr}{\widehat{Corr}}
 \DeclareMathOperator{\hSc}{\widehat{\mathcal{S}}}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\mst}{MST}
\DeclareMathOperator{\supp}{supp}
 \DeclareMathOperator{\dtv}{d_{TV}}
 \DeclareMathOperator{\hdtv}{\hd_{TV}}
 \DeclareMathOperator*{\argmin}{arg\,min}
 \DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\rank}{Rank}
\DeclareMathOperator{\Krank}{Rank_K}
\DeclareMathOperator{\Det}{Det}
\DeclareMathOperator{\poiss}{Poiss}
\DeclareMathOperator{\unif}{Unif} \DeclareMathOperator{\Deg}{Deg}
\def\simiid{{\overset{i.i.d.}{\sim}}}
\def\lcv{{\,\,\underset{cv}{\leq}\,\,}}
\def\gcv{{\,\,\underset{cv}{\geq}\,\,}}
\def\lcx{{\,\,\underset{cx}{\leq}\,\,}}
\def\gcx{{\,\,\underset{cx}{\geq}\,\,}}
\def\leqst{{\,\,\overset{st}{\leq}\,\,}}
\def\geqst{{\,\,\overset{st}{\geq}\,\,}}
\def\eqdist{{\,\,\overset{d}{=}\,\,}}
\def\geqrh{{\,\,\overset{rh}{\geq}\,\,}}
\def\geqlr{{\,\,\overset{lr}{\geq}\,\,}}
\def\eqlr{{\,\,\overset{lr}{=}\,\,}}
\def\comment{{\mbox{\bf Comment\_Anima: }}}
\def\tha{{\mbox{\tiny th}}}

\DeclareMathOperator{\Aug}{Aug}
\DeclareMathOperator{\watts}{Watts}
\DeclareMathOperator{\girth}{Girth}
\DeclareMathOperator{\PL}{PL}
\DeclareMathOperator{\LP}{LP}
\DeclareMathOperator{\ER}{ER}
\DeclareMathOperator{\reg}{Reg}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\hSigma}{\widehat{\Sigma}}
%\DeclareMathOperator{\hrho}{\widehat{\rho}}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Poiss}{Poiss}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\Diam}{Diam}
\def\erf{\mbox{erf}}
\def\erfc{\mbox{erfc}}
\def\qfunc{\mbox{Q}}
%\def\myexp{\mbox{e}}
\def\snr{\mbox{{SNR}}}
\def\signum{\mbox{sgn}}
\def\Card{\mbox{Card}}
\DeclareMathOperator*{\plim}{plim}
\def\convd{\overset{d}\rightarrow}
\def\convp{\overset{p}\rightarrow}
\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\def\pl{{\parallel}}
%\DeclarePairedDelimiter\norm{\lVert}{\rVert}
%\DeclarePairedDelimiter\nuclearnorm{\lVert}{\rVert_*}
%\DeclarePairedDelimiter\onenorm{\lVert}{\rVert_1}
%\def\rinfnorm{\rVert_{\infty}}
%\DeclarePairedDelimiter\infnorm{\lVert}{\rinfnorm}
%\def\lnorm{{\lvert\!\lvert\!\lvert}}
%\def\rnorm{{\rvert\!\rvert\!\rvert}}
%\DeclarePairedDelimiter\gennorm{\lnorm}{\rnorm}
% \DeclarePairedDelimiter\abs{\lvert}{\rvert}
% \DeclarePairedDelimiter\geninfnorm{\lnorm}{\rnorm_{\infty}}
% \DeclarePairedDelimiter\genonenorm{\lnorm}{\rnorm_{1}}
\DeclareMathOperator{\atanh}{atanh}
 \DeclareMathOperator{\sech}{sech}
 \def\0{{\bf 0}}

\DeclareMathOperator{\lea}{\overset{(a)}{\leq}}
\DeclareMathOperator{\leb}{\overset{(b)}{\leq}}
\DeclareMathOperator{\lec}{\overset{(c)}{\leq}}
\DeclareMathOperator{\led}{\overset{(d)}{\leq}}
\DeclareMathOperator{\lee}{\overset{(e)}{\leq}}

\DeclareMathOperator{\eqa}{\overset{(a)}{=}}
\DeclareMathOperator{\eqb}{\overset{(b)}{=}}
\DeclareMathOperator{\eqc}{\overset{(c)}{=}}
\DeclareMathOperator{\eqd}{\overset{(d)}{=}}
\DeclareMathOperator{\eqe}{\overset{(e)}{=}}

\DeclareMathOperator{\gea}{\overset{(a)}{\geq}}
\DeclareMathOperator{\geb}{\overset{(b)}{\geq}}
\DeclareMathOperator{\gec}{\overset{(c)}{\geq}}
\DeclareMathOperator{\ged}{\overset{(d)}{\geq}}
\DeclareMathOperator{\gee}{\overset{(e)}{\geq}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
% \algrenewcommand{\algorithmiccomment}[1]{// #1}
% \algrenewcommand{\algorithmicrequire}{\textbf{Input:}}
% \algrenewcommand{\algorithmicforall}{\textbf{for each}}


%text abbreviations
%\def\etal{{et al. \/}}
\def\viz{{viz.,\ \/}}
\def\ie{{i.e.,\ \/}}
\def\eg{{e.g.,\ \/}}
\def\etc{{etc.  }}
\def\ifff{{iff  }}
\def\as{{a.s.  }}
\def\st{{s.t.  }}
\def\wpone{{w.p.}\,1\,\,}
\def\wpp{{w.p.p.}\,\,}
\def\for{\,\,\mbox{for}\quad}
\def\ifmbox{\,\,\mbox{if}\quad}
\def\nn{\nonumber}
%\def\qed{\hfill$\Box$}
\def\ni{\noindent}

\def\qed{\hfill\hbox{${\vcenter{\vbox{
    \hrule height 0.4pt\hbox{\vrule width 0.4pt height 6pt
    \kern5pt\vrule width 0.4pt}\hrule height 0.4pt}}}$}}
\def\complx{\mathbb{C}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%ldp : use ldp.tex file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Detection on Graphs



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%colors
\def\tcr{\textcolor{red}}
\def\tcb{\textcolor{blue}}
\def\tcg{\textcolor{green}}
\def\tcw{\textcolor{white}}
\def\tcm{\textcolor{magenta}}
\def\tccyan{\textcolor{cyan}}
\def\tcv{\textcolor{violet}}
\definecolor{myred}{rgb}{0.3,0.0,0.7}
\definecolor{dkg}{rgb}{0.1,0.7,0.2}
\definecolor{dkb}{rgb}{0.0,0.2,0.8}

\def\tcdkb{\textcolor{dkb}}
\def\tcdkg{\textcolor{dkg}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\mathscr

\newcommand{\Amsc}{\mathscr{A}}
\newcommand{\Cmsc}{\mathscr{C}}
\newcommand{\Dmsc}{\mathscr{D}}
\newcommand{\Emsc}{\mathscr{E}}
\newcommand{\Fmsc}{\mathscr{F}}
\newcommand{\Gmsc}{\mathscr{G}}
\newcommand{\Hmsc}{\mathscr{H}}
\newcommand{\Kmsc}{\mathscr{K}}
\newcommand{\Nmsc}{\mathscr{N}}
\newcommand{\Pmsc}{\mathscr{P}}
\newcommand{\Qmsc}{\mathscr{Q}}
\newcommand{\Rmsc}{\mathscr{R}}
\newcommand{\Smsc}{\mathscr{S}}
\newcommand{\Tmsc}{\mathscr{T}}
\newcommand{\Umsc}{\mathscr{U}}
\newcommand{\Xmsc}{\mathscr{X}}
\newcommand{\Ymsc}{\mathscr{Y}}



%%%%%%%%%%%%%%%%%%%%%%hat
 \def\ha{\hat{a}}
 \def\hb{\hat{b}}
 \def\hc{\hat{c}}
\def\hd{\widehat{d}}
 \def\he{\widehat{e}}
 \def\hf{\hat{f}}
 \def\hg{\widehat{g}}
 \def\hh{\widehat{h}}
 \def\hi{\widehat{i}}
 \def\hj{\widehat{j}}
 \def\hk{\widehat{k}}
 \def\hl{\widehat{l}}
 \def\hm{\widehat{m}}
 \def\hn{\widehat{n}}
 \def\ho{\widehat{o}}
 \def\hp{\widehat{p}}
 \def\hq{\widehat{q}}
 \def\hr{\widehat{r}}
 \def\hs{\widehat{s}}
 \def\hatt{\widehat{t}}
 \def\hu{\hat{u}}
 \def\hv{\widehat{v}}
 \def\hw{\hat{w}}
 \def\hx{\hat{x}}
 \def\hy{\hat{y}}
 \def\hz{\widehat{z}}
% %bold caps
 \def\hA{\hat{A}}
 \def\hB{\hat{B}}
 \def\hC{\hat{C}}
 \def\hD{\widehat{D}}
 \def\hE{\widehat{E}}
 \def\hF{\widehat{F}}
 \def\hG{\widehat{G}}
 \def\hH{\widehat{H}}
 \def\hI{\widehat{I}}
 \def\hJ{\widehat{J}}
 \def\hK{\widehat{K}}
 \def\hL{\widehat{L}}
 \def\hM{\widehat{M}}
\def\hN{\widehat{N}}
 \def\hO{\widehat{O}}
 \def\hP{\widehat{P}}
 \def\hQ{\widehat{Q}}
 \def\hR{\widehat{R}}
 \def\hS{\widehat{S}}
\def\hT{\widehat{T}}
 \def\hU{\widehat{U}}
 \def\hV{\widehat{V}}
\def\hW{\widehat{W}}
 \def\hX{\hat{X}}
 \def\hY{\widehat{Y}}
 \def\hZ{\widehat{Z}}

 \def\hlambda{\widehat{\lambda}}
\def\hpi{\widehat{\pi}}
\def\hnu{\widehat{\nu}}
\def\hbd{\widehat{\mathbf{d}}}


\def\bLambda{\mathbf{\Lambda}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%bold alphabets
\def\bfzero{{\mathbf{0}}}
\def\bfone{{\mathbf{1}}}
\def\bfa{{\mathbf a}}
\def\bfb{{\mathbf b}}
\def\bfc{{\mathbf c}}
\def\bfd{{\mathbf d}}
\def\bfe{{\mathbf e}}
\def\bff{{\mathbf f}}
\def\bfg{{\mathbf g}}
\def\bfh{{\mathbf h}}
\def\bfi{{\mathbf i}}
\def\bfj{{\mathbf j}}
\def\bfk{{\mathbf k}}
\def\bfl{{\mathbf l}}
\def\bfm{{\mathbf m}}
\def\bfn{{\mathbf n}}
\def\bfo{{\mathbf o}}
\def\bfp{{\mathbf p}}
\def\bfq{{\mathbf q}}
\def\bfr{{\mathbf r}}
\def\bfs{{\mathbf s}}
\def\bft{{\mathbf t}}
\def\bfu{{\mathbf u}}
\def\bfv{{\mathbf v}}
\def\bfw{{\mathbf w}}
\def\bfx{{\mathbf x}}
\def\bfy{{\mathbf y}}
\def\bfz{{\mathbf z}}
%bold caps
\def\bfA{{\mathbf A}}
\def\bfB{{\mathbf B}}
\def\bfC{{\mathbf C}}
\def\bfD{{\mathbf D}}
\def\bfE{{\mathbf E}}
\def\bfF{{\mathbf F}}
\def\bfG{{\mathbf G}}
\def\bfH{{\mathbf H}}
\def\bfI{{\mathbf I}}
\def\bfJ{{\mathbf J}}
\def\bfK{{\mathbf K}}
\def\bfL{{\mathbf L}}
\def\bfM{{\mathbf M}}
\def\bfN{{\mathbf N}}
\def\bfO{{\mathbf O}}
\def\bfP{{\mathbf P}}
\def\bfQ{{\mathbf Q}}
\def\bfR{{\mathbf R}}
\def\bfS{{\mathbf S}}
\def\bfT{{\mathbf T}}
\def\bfU{{\mathbf U}}
\def\bfV{{\mathbf V}}
\def\bfW{{\mathbf W}}
\def\bfX{{\mathbf X}}
\def\bfY{{\mathbf Y}}
\def\bfZ{{\mathbf Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%bold symbols

\def\alphabf{\hbox{\boldmath$\alpha$\unboldmath}}
\def\betabf{\hbox{\boldmath$\beta$\unboldmath}}
\def\gammabf{\hbox{\boldmath$\gamma$\unboldmath}}
\def\deltabf{\hbox{\boldmath$\delta$\unboldmath}}
\def\epsilonbf{\hbox{\boldmath$\epsilon$\unboldmath}}
\def\zetabf{\hbox{\boldmath$\zeta$\unboldmath}}
\def\etabf{\hbox{\boldmath$\eta$\unboldmath}}
\def\iotabf{\hbox{\boldmath$\iota$\unboldmath}}
\def\kappabf{\hbox{\boldmath$\kappa$\unboldmath}}
\def\lambdabf{\hbox{\boldmath$\lambda$\unboldmath}}
\def\mubf{\hbox{\boldmath$\mu$\unboldmath}}
\def\nubf{\hbox{\boldmath$\nu$\unboldmath}}
\def\xibf{\hbox{\boldmath$\xi$\unboldmath}}
\def\pibf{\hbox{\boldmath$\pi$\unboldmath}}
\def\rhobf{\hbox{\boldmath$\rho$\unboldmath}}
\def\sigmabf{\hbox{\boldmath$\sigma$\unboldmath}}
\def\taubf{\hbox{\boldmath$\tau$\unboldmath}}
\def\upsilonbf{\hbox{\boldmath$\upsilon$\unboldmath}}
\def\phibf{\hbox{\boldmath$\phi$\unboldmath}}
\def\chibf{\hbox{\boldmath$\chi$\unboldmath}}
\def\psibf{\hbox{\boldmath$\psi$\unboldmath}}
\def\omegabf{\hbox{\boldmath$\omega$\unboldmath}}
\def\inftybf{\hbox{\boldmath$\infty$\unboldmath}}
\def\hSigmabf{\hbox{$\widehat{\bf \Sigma}$}}
\def\Sigmabf{\hbox{$\bf \Sigma$}}
\def\Upsilonbf{\hbox{$\bf \Upsilon$}}
%\def\Phibf{\hbox{$\bf \Phi$}}
%\def\Psibf{\hbox{$\bf \Psi$}}
\def\Omegabf{\hbox{$\bf \Omega$}}
\def\Deltabf{\hbox{$\bf \Delta$}}
\def\Gammabf{\hbox{$\bf \Gamma$}}
\def\Thetabf{\hbox{$\bf \Theta$}}
\def\Lambdabf{\mbox{$ \bf \Lambda $}}
\def\Xibf{\hbox{\bf$\Xi$}}
\def\Pibf{{\bf \Pi}}
%\def\thetabf{\hbox{\boldmath$\theta$\unboldmath}}
\def\thetabf{{\mbox{\boldmath$\theta$\unboldmath}}}
%\def\thetabf{\hbox{$\bf{\theta}$}}
\def\Upsilonbf{\hbox{\boldmath$\Upsilon$\unboldmath}}
\newcommand{\Phibf}{\mbox{${\bf \Phi}$}}
\newcommand{\Psibf}{\mbox{${\bf \Psi}$}}
\def\olambda{\mathfrak{o}(\lambda)}
\def\complex{\mathfrak{C}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Calligraphic
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
%\def\Pc{{\cal P}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Wc{{\cal W}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%mathbb
\def\Abb{{\mathbb A}}
\def\BBb{{\mathbb B}}% different
\def\Cbb{{\mathbb C}}
\def\Dbb{{\mathbb D}}
\def\Ebb{{\mathbb E}}
\def\Fbb{{\mathbb F}}
\def\Gbb{{\mathbb G}}
\def\Hbb{{\mathbb H}}
\def\Ibb{{\mathbb I}}
\def\Jbb{{\mathbb J}}
\def\Kbb{{\mathbb K}}
\def\Lbb{{\mathbb L}}
\def\Mbb{{\mathbb M}}
\def\Nbb{{\mathbb N}}
\def\Obb{{\mathbb O}}
\def\Pbb{{\mathbb P}}
\def\Qbb{{\mathbb Q}}
\def\Rbb{{\mathbb R}}
\def\Sbb{{\mathbb S}}
\def\Tbb{{\mathbb T}}
\def\Ubb{{\mathbb U}}
\def\Vbb{{\mathbb V}}
\def\Wbb{{\mathbb W}}
\def\Xbb{{\mathbb X}}
\def\Ybb{{\mathbb Y}}
\def\Zbb{{\mathbb Z}}

\def\hbfP{{\widehat{\bfP}}}

\def\tilf{{\widetilde{f}}}

\def\tilo{{\widetilde{o}}}
\def\tilomega{{\widetilde{\omega}}}

\def\tilJbf{{\widetilde{\bfJ}}}

%\def\tilJ{{\widetilde{J}}}
\def\tilO{{\widetilde{O}}}
%\def\tilP{{\widetilde{P}}}
\def\tilR{{\widetilde{R}}}

\def\tilAbf{{\widetilde{\bfA}}}
\def\tilJbf{{\widetilde{\bfJ}}}
\def\tilRbf{{\widetilde{\bfR}}}


\def\tilEbb{{\widetilde{\Ebb}}}
\def\tilPbb{{\widetilde{\Pbb}}}


\def\tiltilEbb{{\widetilde{\widetilde{\Ebb}}}}
\def\tiltilP{{\widetilde{\widetilde{P}}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%command abbreviations
\newcommand{\bprfof}{\begin{proof_of}}
\newcommand{\eprfof}{\end{proof_of}}
\newcommand{\bprf}{\begin{myproof}}
\newcommand{\eprf}{\end{myproof}}
\newcommand{\bp}{\begin{psfrags}}
\newcommand{\ep}{\end{psfrags}}
\newcommand{\bl}{\begin{lemma}}
\newcommand{\el}{\end{lemma}}
\newcommand{\bt}{\begin{theorem}}
\newcommand{\et}{\end{theorem}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bd}{\begin{definition}}
\newcommand{\ed}{\end{definition}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}\noindent}
\def\beqn{\begin{eqnarray}}
\def\eeqn{\end{eqnarray} \noindent}
\def\beqnn{  \begin{eqnarray*}}
\def\eeqnn{\end{eqnarray*}  \noindent}
\def\bcase{  \begin{numcases}}
\def\ecase{\end{numcases}   \noindent}
\def\bsbcase{  \begin{subnumcases}}
\def\esbcase{\end{subnumcases}   \noindent}

\def\endproof{\hfill$\blacksquare$}
\def\defeq{{:=}}%{{\stackrel{\Delta}{=}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%theorems

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{problem}{Problem}
\newtheorem{assumption}{A}
\newtheorem{properties}{Properties}
\newtheorem{conjecture}{Conjecture}
\newtheorem{criterion}{Criterion}
\newtheorem{proposition}{Proposition}
\newtheorem{notation}{Notation}
\newtheorem{derivation}{Derivation}
\newtheorem{claim}{Claim}
\newtheorem{observation}{Observation}
\newtheorem{fact}{Fact}

%\theoremstyle{definition}
\newtheorem{definition}{Definition}
%\theorembodyfont{\upshape} %body not italicized

%\theoremstyle{remark} %Comment it if you want to make the style of remarks the same as theorems
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
%\theoremheaderfont{\normalfont\bfseries}
%\theorembodyfont{\normalfont}
%\newtheorem{example}{Example}
%\newtheorem{proof}{Proof}

\newenvironment{myproof}{\noindent{\bf Proof:} \hspace*{1em}}{
    \hspace*{\fill} $\Box$ }
\newenvironment{proof_of}[1]{\noindent {\bf Proof of #1: }}{\hspace*{\fill} $\Box$ }
\newenvironment{proof_claim}{\begin{quotation} \noindent}{
    \hspace*{\fill} $\diamond$ \end{quotation}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\matplottc}[1]{               % single matlab plot twocolumn
        \unitlength .45truein
        \begin{center}
%         \begin{picture}(5,4.6)(1.05,.45)
        \special{psfile=#1.ps hscale=50 vscale=50}
        \end{picture}
        \end{center}
}
\newcommand{\matplotfp}[1]{               % single matlab plot fullpage
        \unitlength .45truein
        \begin{center}
        \begin{picture}(14,16)(.8,-1)
        \special{psfile=#1.ps hscale=100 vscale=100}
        \end{picture}
        \end{center}
}
\newcommand{\matplothp}[1]{               % single matlab plot halfpage
        \unitlength .45truein
        \begin{center}  \begin{picture}(14,7.5)(-1,.55)
        \special{psfile=#1.ps hscale=80 vscale=80}
        \end{picture}
        \end{center}
}
\newcommand{\matplothptop}[1]{               % single matlab plot halfpage
        \unitlength .45truein                % when figure is top of page
        \begin{center}  \begin{picture}(14,6.3)(-1,1.15)
        \special{psfile=#1.ps hscale=80 vscale=80}
        \end{picture}
        \end{center}
}
\newcommand{\matplotcc}[4]{             % two axis('square') plots side by side
        \vspace{2.8in}
        \special{psfile=#1.ps voffset=-10 hoffset=-22 vscale=52 hscale=52}
        \special{psfile=/user/xu/isl/matlab/psfiles/#2.ps voffset=-10 hoffset=213 vscale=52 hscale=52}
        \hspace*{\fill}\hspace*{0.35in}#3\hspace*{\fill}\hspace*{\fill}\hspace*{
0.35in}#4\hspace*{\fill} }
\newcommand{\matplottwo}[4]{             % two axis('normal') plots side by side
        \vspace{2.62in}
        \special{psfile=#1.ps voffset=-10 hoffset=-27 vscale=52 hscale=52}
        \special{psfile=#2.ps voffset=-10 hoffset=218 vscale=52 hscale=52}
        \vspace*{0.18in}
        \hspace*{\fill}\hspace*{-.05in}#3\hspace*{\fill}\hspace*{\fill}\hspace*{
0.65in}#4\hspace*{\fill} } %%
%% This is for making fancy paragraphs
%%
\def\psfancypar#1#2{\begingroup\def\par{\endgraf\endgroup\lineskiplimit=0pt}
               \setbox2=\hbox{\large\sc #2}
%              \showthe\lht2\showthe\baselineskip
               \newdimen\tmpht \tmpht \ht2 \advance\tmpht by \baselineskip
%              \showthe\tmpht
% Changed 10/2/89 rhr - t-bol -> Times-Bold for dvi2ps to dvips conversion
%              \font\hhuge=t-bol at \tmpht
               \font\hhuge=Times-Bold at \tmpht
               \setbox1=\hbox{{\hhuge #1}}
%              \showthe\ht1
               \count7=\tmpht \count8=\ht1
%  note that all this BS is necessary since TeX only does integer
%  divides and rounds all results
               \divide\count8 by 1000 \divide\count7 by \count8
%               \showthe\count7
               \tmpht=.001\tmpht\multiply\tmpht by \count7
%               \showthe\tmpht
%              \font\hhuge=t-bol at \tmpht
               \font\hhuge=Times-Bold at \tmpht
               \setbox1=\hbox{{\hhuge #1}}
               \noindent
                \hangindent1.05\wd1
               \hangafter=-2 {\hskip-\hangindent
               \lower1\ht1\hbox{\raise1.0\ht2\copy1}%
                \kern-0\wd1}\copy2\lineskiplimit=-1000pt}


\newenvironment{ap}{
\renewcommand{\thesection}{\mbox{Appendix }\Alph{section}}
\renewcommand{\thesubsection}{\Alph{section}.\arabic{subsection
}}
\renewcommand{\theequation}{\mbox{\Alph{section}.}\arabic{equation}}
}{
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\theequation}{\arabic{equation}}
}



\def\Kout{\setbox1=\hbox{\Huge\bf K}\hbox to
1.05\wd1{\hspace{.05\wd1}\special{
"/Times-BoldItalic findfont 25 scalefont setfont
/prKzip
{0 0 moveto (K) show} def
/dozip
{gsave
  /xp 0 def
  .08 -.04 0
  {
   setgray
  prKzip
%  /xp xp dx add def xp -.7 translate %for
  -.7 .4 translate} for
  1 setgray prKzip
  0 0 moveto
  0 setgray
  .5 setlinewidth
  (K) true charpath  stroke
 grestore
} def
dozip}}}
\def\Sout{\setbox1=\hbox{\Huge\bf S}\hbox to 1.05\wd1{\hspace{.05\wd1}\special{"
/Times-BoldItalic findfont 25 scalefont setfont
/prSzip
{0 0 moveto (S) show} def
/dozip
{gsave
  /xp 0 def
  .08 -.04 0
  {
   setgray
  prSzip
%  /xp xp dx add def xp -.7 translate %for
  -.7 .4 translate} for
  1 setgray prSzip
  0 0 moveto
  0 setgray
  .5 setlinewidth
  (S) true charpath  stroke
 grestore
} def
dozip}}}
\newcommand{\hKbf}{\mbox{${\widehat{\bfK}}$}}
\newcommand{\hthetabf}{\mbox{${\widehat{\thetabf}}$}}
\newcommand{\hmubf}{\mbox{${\widehat{\mubf}}$}}
%\newcommand{\thbar}{\mbox{${\bar{\thetabf}}_N$}}
%\newcommand{\etahat}{\mbox{${\hat{\etabf}}$}}
%\newcommand{\etabf}{\mbox{${\bf\eta}$}}
%\newcommand{\e}{\mbox{${\bf e}_k$}}
%\newcommand{\ehat}{\mbox{$\hat{\bf e}_k$}}
%\newcommand{\EWE}{\mbox{${\bf E}_s^{}{\bf WE}_s^*$}}
%\newcommand{\DPD}{\mbox{$\Dbf^*\Pbf_{\bf A}^{\perp} \Dbf$}}
%\newcommand{\EWEhat}{\mbox{$\hat{\bf E}_s^{}{\bf W}\hat{\bf E}_s^*$}}
%\newcommand{\E}{\mbox{{\rm E}}}
%\newcommand{\Efs}{\mbox{${\bf E}_s^{}$}}
%\newcommand{\En}{\mbox{${\bf E}_n^{}$}}
%\newcommand{\Eshat}{\mbox{$\hat{\bf E}_s^{}$}}
%\newcommand{\Lshat}{\mbox{$\hat {\bf \Lambda}_s^{}$}}
%\newcommand{\Ls}{\mbox{$ {\bf \Lambda}_s^{}$}}
%\newcommand{\Ln}{\mbox{$ {\bf \Lambda}_n^{}$}}
%\newcommand{\Ltilde}{\mbox{$\widetilde {\bf \Lambda}$}}
%\newcommand{\Enhat}{\mbox{$\hat{\bf E}_n^{}$}}
%\newcommand{\Lnhat}{\mbox{$\hat {\bf \Lambda}_n^{}$}}
%\newcommand{\Ai}{\mbox{$ ({\bf A}^*{\bf A})^{-1} $}}
%\newcommand{\abf}{\mbox{${\bf a}$}}


%Define affiliation at footnote
% Make \small be smaller (8 pt)
%\def\small{\@setsize\small{9pt}\viiipt\@viiipt\let\@listi\@listI}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros to restate theorems in appendices
%
% Use as follows:
%\torestate{Theorem}{thm:restate}{If $x \in \N$ then $x+1 \in \N$.}
%
%\restate{thm:restate}

\newcommand{\torestate}[3]{%
\expandafter \def \csname BBRESTATE #2 \endcsname{#3}
\theoremstyle{plain}
\newtheorem{BBRESTATETHMNUM#2}[theorem]{#1}
\begin{BBRESTATETHMNUM#2}\label{#2}\csname BBRESTATE #2 \endcsname   \end{BBRESTATETHMNUM#2}
\newtheorem*{BBRESTATETHMNONNUM#2}{{#1}~\ref{#2}}
}


\newcommand{\restate}[1]{\begin{BBRESTATETHMNONNUM#1}[Restated] \csname BBRESTATE #1 \endcsname
\end{BBRESTATETHMNONNUM#1}}


\definecolor{blue1}{HTML}{0066FF}
\definecolor{lpurple}{cmyk}{.05,0.18,0,0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> maintable.tex <==
\section{Table of Content}

\begin{table}[htbp]\vspace{-1cm}\caption{Table of Notation My Research}
\begin{center}% used the environment to augment the vertical space
% between the caption and the table
\begin{tabular}{r c p{10cm} }
\toprule

$\X$ &  & Finite state space \\
$\Y$ &  & Finite observation space\\ 
$\A$ &  & Finite action space \\  
$\R$ &  & Finite reward space\\  
$X$ &  & Cardinality of state space\\  
$Y$ &  & Cardinality of observation space\\  
$A$ &  & Cardinality of action space\\  
$R$ &  & Cardinality of reward space\\  
$r_{\max}$ &  & Largest reward\\  
$x$ &  & state indicator random variable\\  
$\vec{y}$ &  & observation indicator random variable\\  
$r$ &  & reward indicator random variable\\
$a~or~l$ &  & action indicator random variable\\    
$T$ &  & Transition tensor \\  
$O$ &  & Observation matrix\\  
$\Gamma$ &  & Reward tensor\\
$\Pi$ &  & Policy matrix\\
$M$ &  & POMDP model\\
$\M^{(k)}$ &  & Set of plausible POMDP at episode $k$\\
$f_T(x'|x,a)$ &  & transition density from state $x$ to state $x'$ given action $a$\\  
$f_O(\vec{y}|x)$ &  & observation density\\  
$f_R(r|x,a)$ &  & reward density given pair of state-action\\  
$f_T(x'|x)$ &  & corresponding Markov chain transition density\\  
$\calP$ &  & Set of all plausible stochastic memory-less policies\\  
$\pi$ &  & memory less policy, observation $\rightarrow$ action\\  
$\pi_{\min}$ &  & smallest element of policy matrix memory-less policy, observation $\rightarrow$ action\\  
$\eta(\pi,M)$ &  & expected average reward given model and policy\\    
$\omega_\pi$ &  & vector of stationary distribution over states given policy $\pi $ \\  
$\vec{v}_{i,t}^{(l)}$ &  & $i'th$ view at time t give $a_t=l$(middle action= $l$), $i\in\{1,2,3\}$\\  
$V_{\nu}^{(l)}$ &  & $\nu'th$ View matrix representation $\nu\in\{1,2,3\}$\\  
$K_{\nu,\nu'}^{(l)}$ &  & Covariance matrix between view $\nu$ and $\nu'$, where $\nu,nu'\in\{1,2,3\}$ given middle action $l$\\  
$M_2^{(l)}$ &  & Second order moment given middle action $l$\\  
$M_3^{(l)}$ &  & Third order moment given middle action $l$\\
$\sigma_{\nu,\nu'}^{(l)}$ &  & smallest non-zero singular value of covariance matrix of views $\nu$ and $\nu'$ given middle action $l$ \\  
$C_O, C_R, C_T$ &  & Suitable numerical constants\\  
$N$ &  & Number of total samples\\  
$N(l)$ &  & Number of triple with middle action $l$\\    
$D$ &  & The model diameter\\
$\B_O$ &  & Upper confidence bound over error of estimated $f_O$\\  
$\B_R$ &  & Upper confidence bound over error of estimated $f_R$\\  
$\B_T$ &  & Upper confidence bound over error of estimated $f_T$\\

\bottomrule
\end{tabular}
\end{center}
\label{tab:TableOfNotationForMyResearch}
\end{table}


